A search for cool molecular gas in GK Persei and other classical novae

Detecting molecular line emission from classical nova remnants has the potential of revealing information on the composition of the ejecta, in particular, it can deliver accurate isotopic ratios in the matter processed by a thermonuclear runaway. We conducted searches toward more than 100 classical novae for emission in lines of the CO or HCN molecules using single-dish telescopes and interferometric arrays at millimeter and submillimeter wavelengths. The survey demonstrates that classical novae, young or old, are not strong sources of molecular emission at submillimeter and millimeter wavelengths. Additionally, we mapped CO emission around Nova Persei 1901 (GK Per), earlier claimed to be circumstellar in origin. Our measurements indicate that the observed emission is from the interstellar medium. Although no molecular emission at millimeter and submillimeter wavelengths has been found in classical novae, it is still likely that some will be detected with high-sensitivity interferometers such as ALMA.

==> tab-co.tex <==
       & \multicolumn{4}{c}{rms (mK)}\\
       & \multicolumn{2}{c}{WILMA}&\multicolumn{2}{c}{FTS}\\
Object &  LSB &  USB &  LSB &  USB\\
\midrule
V* BC Cas  &  2.23  &  3.64\\
V* CP Lac  &  2.28  &  3.47\\
V* DI Lac  &  2.13  &  3.12\\
V* V630 Cas   &  1.62  &  2.28\\
V* V723 Cas   &  2.03  &  2.88\\
NOVA Per 1887  &  2.17  &  2.95\\


==> tab-hcn.tex <==
Object &\multicolumn{2}{c}{rms (mK)}\\ 
       &HCN(1--0) &  HCN(1--0)\,USB\\
\midrule
V* BC Cas  &  4.26  &  5.25\\
NOVA Aql 1917   &  3.83  &  4.51\\
V* CI Gem  &  4.76  &  5.74\\
V* CK Vul  &  7.10  &  8.33\\
V* CP Lac  &  3.29  &  4.03\\
V* DI Lac  &  4.08  &  4.64\\
NOVA Gem 1903   &  3.93  &  5.05\\
V* DN Gem  &  3.87  &  4.81\\
NOVA Ser 1960   &  7.29  &  8.44\\
V* EL Aql  &  3.90  &  4.11\\
V* GK Per  &  2.61  &  2.80\\
NOVA Ori 1916   &  6.24  &  7.75\\
NOVA Sge 1977   &  4.74  &  5.72\\
NOVA Mon 1942   &  5.54  &  6.63\\
NOVA And 1986   &  3.38  &  4.06\\
V* PQ And  &  2.40  &  2.85\\
V* Q Cyg  &  3.24  &  3.60\\
V* RS Oph  &  6.71  &  8.48\\
NOVA UMi 1956   &  5.21  &  6.11\\
NOVA Sge 1916   &  4.56  &  5.84\\
NOVA Gem 1857   &  4.15  &  5.30\\
NOVA Per 1853   &  2.58  &  2.79\\
V* UW Per  &  3.14  &  3.62\\
V* UZ Tri  &  5.59  &  6.57\\
V* V1059 Sgr    &  3.50  &  3.83\\
V* V1229 Aql    &  4.01  &  4.71\\
V* V1378 Aql    &  3.97  &  4.48\\
V* V1449 Cyg    &  3.30  &  4.17\\
V* V1500 Cyg    &  3.20  &  3.70\\
NOVA Cyg 1978   &  3.30  &  3.94\\
V* V1697 Cyg    &  3.39  &  3.77\\
V* V1974 Cyg    &  3.41  &  4.03\\
NOVA Oph 1994   &  7.53  &  9.25\\
NOVA Cyg 2005   &  3.36  &  3.94\\
NOVA Cyg 2006   &  3.11  &  4.23\\
V* V2467 Cyg    &  3.23  &  3.89\\
PN K 3-25  &  2.78  &  3.45\\
NOVA Her 1892   &  9.47  &  11.77\\
V* V368 Aql  &  4.57  &  5.67\\
NOVA Per 1974   &  3.20  &  3.73\\
V* V446 Her  &  3.46  &  4.11\\
NOVA Cyg 1948   &  2.36  &  2.87\\
V* V476 Cyg  &  3.43  &  4.10\\
NOVA Aql 1943   &  4.54  &  5.89\\
NOVA Ori 1667   &  4.17  &  5.47\\
HD 176779  &  3.69  &  4.39\\
HD 181419  &  4.03  &  4.41\\
V* V630 Cas  &  4.37  &  4.59\\
V* V705 Cas  &  3.31  &  4.10\\
V* V723 Cas  &  3.75  &  4.75\\
NOVA Her 1991   &  3.53  &  4.11\\
V* V838 Mon  &  1.44  &  1.89\\
NOVA Aql 1951   &  3.62  &  3.79\\
NOVA Oph 1919   &  17.22  &  20.94\\
NOVA Per 1887   &  4.13  &  4.87\\
V* VY Aqr  &  2.65  &  3.18\\
NOVA Gem 1856   &  3.63  &  4.19\\
NOVA Ari 1855   &  2.69  &  2.92\\
NOVA Sge 1783   &  4.73  &  5.67\\

